An Introduction to Space-Time Exterior Calculus

The basic concepts of exterior calculus for space-time multivectors are presented: interior and exterior products, interior and exterior derivatives, oriented integrals over hypersurfaces, circulation and flux of multivector fields. Two Stokes theorems relating the exterior and interior derivatives with circulation and flux respectively are derived. As an application, it is shown how the exterior-calculus space-time formulation of the electromagnetic Maxwell equations and Lorentz force recovers the standard vector-calculus formulations, in both differential and integral forms.

==> preamble.tex <==
\usepackage{amsmath,amsthm}
\usepackage{amssymb}
\usepackage{amstext}
\usepackage{graphicx}
%\usepackage{lscape}
\usepackage{stmaryrd}
%\usepackage{lmodern}

\usepackage{color}
\usepackage[applemac]{inputenc}

\usepackage{pict2e}

%% for plots
\usepackage{tikz}
\usetikzlibrary{shapes}
\usetikzlibrary{positioning}
%% for subfigures
\usepackage{subcaption}
%\usepackage[linkcolor=gray,citecolor=blue,urlcolor=blue]{hyperref}

\makeatletter
\DeclareRobustCommand{\lintprod}{%
  \mathbin{\mathpalette\int@prod{(0,0)(0.8,0)(0.8,0.8)}}%
}
\DeclareRobustCommand{\rintprod}{%
  \mathbin{\mathpalette\int@prod{(0.1,0.8)(0.1,0)(0.9,0)}}}

\newcommand{\int@prod}[2]{%
  \begingroup
  \sbox\z@{$\m@th#1+$}%
  \setlength\unitlength{\wd\z@}%
  \linethickness{0.09\unitlength}%
  \begin{picture}(1,1)
  \roundcap
  \polyline#2
  \end{picture}%
  \endgroup
}
\makeatother

%\renewcommand{\rintprod}{\lrcorner}

\usepackage[justification=centerlast]{caption}%subfig
\usepackage[retainorgcmds]{IEEEtrantools}

\newcommand{\Ab}{{\mathbf A}}
\newcommand{\Bb}{{\mathbf B}}
\newcommand{\Db}{{\mathbf D}}
\newcommand{\Eb}{{\mathbf E}}
\newcommand{\Fb}{{\mathbf F}}
\newcommand{\Gb}{{\mathbf G}}
\newcommand{\Hb}{{\mathbf H}}
\newcommand{\Jb}{{\mathbf J}}
\newcommand{\Lb}{{\mathbf L}}
\newcommand{\Mb}{{\mathbf M}}
\newcommand{\Pb}{{\mathbf P}}
\newcommand{\Rb}{{\mathbf R}}
\newcommand{\Sb}{{\mathbf S}}
\newcommand{\Tb}{{\mathbf T}}
\newcommand{\ebf}{{\mathbf e}}
\newcommand{\etbf}{\tilde{\mathbf e}}
\newcommand{\fb}{{\mathbf f}}
\newcommand{\ftb}{\tilde{\mathbf f}}
\newcommand{\fbit}{\pmb{\mathit f}}
\newcommand{\jb}{{\mathbf j}}
\newcommand{\kb}{{\mathbf k}}
\newcommand{\pb}{{\mathbf p}}
\newcommand{\xb}{{\mathbf x}}
\newcommand{\yb}{{\mathbf y}}
\newcommand{\ub}{{\mathbf u}}
\newcommand{\vb}{{\mathbf v}}
\newcommand{\wb}{{\mathbf w}}

\newcommand{\drm}{\,\mathrm{d}}

\newcommand{\myparallel}{{\mkern3mu\vphantom{\perp}\vrule depth 0pt\mkern3mu\vrule depth 0pt\mkern3mu}}

\newcommand{\deltabf}{{\boldsymbol \partial}}
\newcommand{\Omegabf}{{\boldsymbol \Omega}}
\newcommand{\omegabf}{{\boldsymbol \omega}}

\def\kbar{{\mathchar'25\mkern-9mu k}}
\def\kbfbar{{\mathchar'26\mkern-9mu \kb}}

\newcommand{\mf}{{\mathbf F}}
\newcommand{\sd}{{\mathbf J}}
\newcommand{\vp}{{\mathbf A}}
\newcommand{\gf}{{\mathbf G}}

\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\sgn}{sgn}

\newcommand{\vabs}[1]{\lvert#1\rvert}
\newcommand{\len}[1]{\lvert#1\rvert}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\hodge}{{\scriptscriptstyle\mathcal{H}}}
\newcommand{\hodgeinv}{{\scriptscriptstyle\mathcal{H}^{-1}}}

\newcommand{\overdot}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}

\newtheoremstyle{question}
  {\topsep}   % ABOVESPACE
  {\topsep}   % BELOWSPACE
  {\upshape}  % BODYFONT
  {0pt}       % INDENT (empty value is the same as 0pt)
  {\itshape}  % HEADFONT
  {.}         % HEADPUNCT
  {5pt plus 1pt minus 1pt} % HEADSPACE
  {\thmname{#1} \thesection.\thmnumber{\itshape#2}\thmnote{(#3)}} % CUSTOM-HEAD-SPEC

\makeatletter
    \def\@endtheorem{\hfill$\P$\endtrivlist\@endpefalse }
\makeatother
\theoremstyle{question}
\theoremstyle{remark}
\theoremstyle{definition}
\newtheorem{Question}{Question}
\newtheorem{Example}{Example}



\settrimmedsize{297mm}{210mm}{*}
\setlength{\trimtop}{0pt}
\setlength{\trimedge}{\stockwidth}
\addtolength{\trimedge}{-\paperwidth}
\settypeblocksize{664pt}{498.13pt}{*}
\setulmargins{3cm}{*}{*}
\setlrmargins{*}{*}{0.75}
\setmarginnotes{17pt}{51pt}{\onelineskip}
\setheadfoot{\onelineskip}{2\onelineskip}
\setheaderspaces{*}{2\onelineskip}{*}
\checkandfixthelayout

\renewcommand{\chapterheadstart}{\newpage}
\renewcommand{\printchaptername}{}
\renewcommand{\chapnumfont}{\normalfont}
%\renewcommand{\chapternamenum}{}
%\renewcommand{\printchapternum}{\thechapter}
%\renewcommand{\afterchapternum}{}
\renewcommand{\printchaptertitle}[1]{%
  \raggedright\Large\scshape\MakeLowercase{#1}}
\renewcommand{\afterchaptertitle}{%
       \vskip\onelineskip}% \hrule\vskip\onelineskip}
\setsecheadstyle{\raggedright\scshape\MakeLowercase}
\setbeforesecskip{-\onelineskip}
\setaftersecskip{\onelineskip}
\setsubsecheadstyle{\sethangfrom{\noindent ##1}\raggedright\itshape}
\setbeforesubsecskip{-\onelineskip}
\setaftersubsecskip{\onelineskip}

\pagestyle{plain}

\author{\scshape Ivano Colombaro, Josep Font-Segura, Alfonso Martinez}

\date{\scshape\MakeLowercase\today}

\renewcommand{\abstractnamefont}{\scshape\MakeLowercase}

\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother
